Are VLMs Ready for Autonomous Driving? An Empirical Study from the Reliability, Data, and Metric Perspectives

Recent advancements in Vision-Language Models (VLMs) have sparked interest in their use for autonomous driving, particularly in generating interpretable driving decisions through natural language. However, the assumption that VLMs inherently provide visually grounded, reliable, and interpretable explanations for driving remains largely unexamined. To address this gap, we introduce DriveBench, a benchmark dataset designed to evaluate VLM reliability across 17 settings (clean, corrupted, and text-only inputs), encompassing 19,200 frames, 20,498 question-answer pairs, three question types, four mainstream driving tasks, and a total of 12 popular VLMs. Our findings reveal that VLMs often generate plausible responses derived from general knowledge or textual cues rather than true visual grounding, especially under degraded or missing visual inputs. This behavior, concealed by dataset imbalances and insufficient evaluation metrics, poses significant risks in safety-critical scenarios like autonomous driving. We further observe that VLMs struggle with multi-modal reasoning and display heightened sensitivity to input corruptions, leading to inconsistencies in performance. To address these challenges, we propose refined evaluation metrics that prioritize robust visual grounding and multi-modal understanding. Additionally, we highlight the potential of leveraging VLMs' awareness of corruptions to enhance their reliability, offering a roadmap for developing more trustworthy and interpretable decision-making systems in real-world autonomous driving contexts. The benchmark toolkit is publicly accessible.

==> tables/corruption_params.tex <==
\begin{table}[t]
    \centering
    \caption{Severity level setups in corruption simulations: Detailed parameters used for generating multi-level corruptions for each corruption type.}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c}
        \toprule
        \textbf{Corruption} & \textbf{Parameter} & \textbf{Value} 
        \\\midrule\midrule
        \rowcolor{gray!10}Bright & adjustment in HSV space &
        \\
        Dark & scale factor &
        \\
        \rowcolor{gray!10}Fog & (thickness, smoothness) &
        \\
        Snow & \makecell{(mean, std, scale, threshold, \\blur radius, blur std, blending ratio)} &
        \\
        Rain &  &
        \\
        Water &  &
        \\
        Lens &  &
        \\
        \rowcolor{gray!10}Crash & number of dropped camera & 
        \\
        Frame & probability of frame dropping  & 
        \\
        Saturate &   & 
        \\
        \rowcolor{gray!10}Motion & (radius, sigma) & 
        \\
        \rowcolor{gray!10}Zoom & (radius, sigma) & 
        \\
        \rowcolor{gray!10}Zoom & (radius, sigma) & 
        \\
        Quant & bit number &
        \\
        \bottomrule
    \end{tabular}}
    \label{tab:my_label}
\end{table}

==> tables/detector.tex <==
\begin{table}[t]
    \centering
    \caption{Performance under various corruptions and after denoising. Each corruption has two sub-columns: performance under corruption and performance after denoising using the VLM agent.}
    \vspace{-0.2cm}
    \label{tab:detector}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|cccc}
    \toprule
    \textbf{Method} & \textbf{NDS} & \textbf{mCE} & \textbf{mRR} 
    \\\midrule\midrule
    DETR3D~\cite{wang2022detr3d}  
    \\
    BEVFormer~\cite{li2022bevformer} 
    \\
    \bottomrule
    \end{tabular}}
\end{table}

==> tables/drivelm_dist_behavior.tex <==
\begin{table}[t]
    \centering
    \caption{Behavior MCQ choice: the question asks about the behavior of ego vehicles considering steer and speed.}
    \vspace{-0.1cm}
    \label{tab:drivelm-behavior-dist}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|c|c|c|c|c}
    \toprule
    Speed \textbackslash Steer & Left & Slightly Left & Going Straight & Slightly Right & Right \\\midrule
    Very Fast & 2 & 5 & 119 & 13 & 0 \\
    Fast & 1 & 17 & 189 & 15 & 6 \\
    Normal Speed & 10 & 15 & 78 & 27 & 9 \\
    Snow & 9 & 14 & 107 & 18 & 10 \\
    Not Moving & 0 & 0 & 135 & 0 & 0 \\
    \bottomrule
    \end{tabular}}
\end{table}

==> tables/drivelm_dist_perception.tex <==
\begin{table}[t]
    \centering
    \caption{Perception MCQ choice: the question asks about the moving status of surrounding vehicles with given coordinates.}
    \vspace{-0.1cm}
    \label{tab:drivelm-percept-dist}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{r|ccccc}
    \toprule
    Data &Going ahead & Turn left & Turn right & Drive backward & Reverse parking
    \\\midrule
    Train &\textbf{3374} & 161 & 145 & 3 & 1\\
    Val & \textbf{695} & 29 & 19 & 1 & 0\\
    \bottomrule
    \end{tabular}}
\end{table}
